A Reanalysis of the Composition of K2-106b: an Ultra-short Period Super-Mercury Candidate

We present a reanalysis of the K2-106 transiting planetary system, with a focus on the composition of K2-106b, an ultra-short period, super-Mercury candidate. We globally model existing photometric and radial velocity data and derive a planetary mass and radius for K2-106b of $M_{p} = 8.53\pm1.02~M_{\oplus}$ and $R_{p} = 1.71^{+0.069}_{-0.057}~R_{\oplus}$, which leads to a density of $\rho_{p} = 9.4^{+1.6}_{-1.5}$ $\rm g~cm^{-3}$, a significantly lower value than previously reported in the literature. We use planet interior models that assume a two-layer planet comprised of a liquid, pure Fe core and iron-free, $\rm MgSiO_{3}$ mantle, and we determine the range of core mass fractions that are consistent with the observed mass and radius. We use existing high-resolution spectra of the host star to derive Fe/Mg/Si abundances ([Fe/H]$=-0.03 \pm 0.01$, [Mg/H]$= 0.04 \pm 0.02$, [Si/H]$=0.03 \pm 0.06$) to infer the composition of K2-106b. We find that although K2-106b has a high density and core mass fraction ($44^{+12}_{-15}\%$) compared to the Earth ($33\%$), its composition is consistent with what is expected assuming that it reflects the relative refractory abundances of its host star. K2-106b is therefore unlikely to be a super-Mercury, as has been suggested in previous literature.

==> EXOFAST_Stellar.tex <==
\begin{table}
\scriptsize
\setlength{\tabcolsep}{2pt}

\centering
\caption{Median values and 68\% confidence interval for global model of K2-106}
\begin{tabular}{llcccc}
  \hline
  \hline
Parameter & Units & Values & & & \\
\hline
\multicolumn{2}{l}{Stellar Parameters:}&\smallskip\\
~~~~$M_*$\dotfill &Mass (\msun)\dotfill &$1.460^{+0.055}_{-0.059}$\\
~~~~$R_*$\dotfill &Radius (\rsun)\dotfill &$1.506\pm0.022$\\
~~~~$L_*$\dotfill &Luminosity (\lsun)\dotfill &$3.67^{+0.16}_{-0.15}$\\
~~~~$\rho_*$\dotfill &Density (cgs)\dotfill &$0.603^{+0.032}_{-0.033}$\\
~~~~$\log{g}$\dotfill &Surface gravity (cgs)\dotfill &$4.247^{+0.019}_{-0.021}$\\
~~~~$T_{\rm eff}$\dotfill &Effective Temperature (K)\dotfill &$6509^{+50}_{-49}$\\
~~~~$[{\rm Fe/H}]$\dotfill &Metallicity (dex)\dotfill &$0.186^{+0.077}_{-0.076}$\\
~~~~$[{\rm Fe/H}]_{0}^\dagger$\dotfill &Initial Metallicity \dotfill &$0.284^{+0.059}_{-0.058}$\\
~~~~$Age$\dotfill &Age (Gyr)\dotfill &$0.78^{+0.61}_{-0.42}$\\
~~~~$EEP^\ddagger$\dotfill &Equal Evolutionary Point \dotfill &$323^{+16}_{-23}$\\
~~~~$vsinI_*$\dotfill &Projected rotational velocity (km/s)\dotfill &$19.76\pm0.160$\\
~~~~$\xi$\dotfill &Macroturbulence velocity (km/s)\dotfill &$5.76^{+0.51}_{-0.50}$\\
\hline
\end{tabular}
\begin{flushleft} 
  \footnotesize{ 
    \textbf{\textsc{NOTES:}}
$^\dagger$The initial metallicity is the metallicity of the star when it was formed.\\
$^\ddagger$The Equal Evolutionary Point corresponds to static points in a stars evolutionary history when using the MIST isochrones and can be a proxy for age. See \S2 in \citet{Dotter:2016} for a more detailed description of EEP.
               }
 \end{flushleft}
\label{tab:exofast_stellar}
\end{table}
